EfficientTrain++: Generalized Curriculum Learning for Efficient Visual Backbone Training

The superior performance of modern visual backbones usually comes with a costly training procedure. We contribute to this issue by generalizing the idea of curriculum learning beyond its original formulation, i.e., training models using easier-to-harder data. Specifically, we reformulate the training curriculum as a soft-selection function, which uncovers progressively more difficult patterns within each example during training, instead of performing easier-to-harder sample selection. Our work is inspired by an intriguing observation on the learning dynamics of visual backbones: during the earlier stages of training, the model predominantly learns to recognize some 'easier-to-learn' discriminative patterns in the data. These patterns, when observed through frequency and spatial domains, incorporate lower-frequency components, and the natural image contents without distortion or data augmentation. Motivated by these findings, we propose a curriculum where the model always leverages all the training data at every learning stage, yet the exposure to the 'easier-to-learn' patterns of each example is initiated first, with harder patterns gradually introduced as training progresses. To implement this idea in a computationally efficient way, we introduce a cropping operation in the Fourier spectrum of the inputs, enabling the model to learn from only the lower-frequency components. Then we show that exposing the contents of natural images can be readily achieved by modulating the intensity of data augmentation. Finally, we integrate these aspects and design curriculum schedules with tailored search algorithms. The resulting method, EfficientTrain++, is simple, general, yet surprisingly effective. It reduces the training time of a wide variety of popular models by 1.5-3.0x on ImageNet-1K/22K without sacrificing accuracy. It also demonstrates efficacy in self-supervised learning (e.g., MAE).

==> PaperForReview.tex <==
% % CVPR 2023 Paper Template
% % based on the CVPR template provided by Ming-Ming Cheng (https://github.com/MCG-NKU/CVPR_Template)
% % modified and extended by Stefan Roth (stefan.roth@NOSPAMtu-darmstadt.de)

% \documentclass[10pt,twocolumn,letterpaper]{article}

% %%%%%%%%% PAPER TYPE  - PLEASE UPDATE FOR FINAL VERSION
% % \usepackage[review]{cvpr}      % To produce the REVIEW version
% % \usepackage{cvpr}              % To produce the CAMERA-READY version
% \usepackage[pagenumbers]{cvpr} % To force page numbers, e.g. for an arXiv version

% % Include other packages here, before hyperref.
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}

% % It is strongly recommended to use hyperref, especially for the review version.
% % hyperref with option pagebackref eases the reviewers' job.
% % Please disable hyperref *only* if you encounter grave issues, e.g. with the
% % file validation for the camera-ready version.
% %
% % If you comment hyperref and then uncomment it, you should delete
% % ReviewTempalte.aux before re-running LaTeX.
% % (Or just hit 'q' on the first LaTeX run, let it finish, and you
% %  should be clear).
% \usepackage[pagebackref,breaklinks,colorlinks]{hyperref}

% \usepackage[table]{xcolor}

% \usepackage{xcolor}
% \usepackage{bm}
% \usepackage{bbding}
% \usepackage{amsmath}
% \usepackage{algorithmic}
% \usepackage{algorithm}
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage{wrapfig}
% \usepackage{amsthm}
% \usepackage{caption}
% \usepackage{subcaption}
% \usepackage{pifont}% http://ctan.org/pkg/pifont
% \newcommand{\cmark}{\ding{51}}%
% \newcommand{\xmark}{\ding{55}}%

% \usepackage{hhline}
% \usepackage{enumitem}
% \usepackage{lipsum}
% \setlist[itemize]{leftmargin=*}
% % \usepackage{showframe}
% % \usepackage{enumitem}

% % Support for easy cross-referencing
% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}


% %%%%%%%%% PAPER ID  - PLEASE UPDATE
% \def\cvprPaperID{1166} % *** Enter the CVPR Paper ID here
% \def\confName{CVPR}
% \def\confYear{2023}



% \newtheorem{proposition}{Proposition}
% \newtheorem{lemma}{Lemma}
% % \newtheorem*{proposition_1}{Proposition 1}
% \renewcommand{\proofname}{\textbf{Proof}}


% \definecolor{baselinecolor}{gray}{.9}
% \newcommand{\baseline}[1]{\cellcolor{baselinecolor}{#1}}
% \newlength\savewidth\newcommand\shline{\noalign{\global\savewidth\arrayrulewidth
%   \global\arrayrulewidth 1.25pt}\hline\noalign{\global\savewidth\arrayrulewidth
%   \global\arrayrulewidth 0.575pt}}

% \begin{document}


% %%%%%%%%% TITLE - PLEASE UPDATE
% \title{EfficientTrain: Exploring Generalized Curriculum Learning\\for Training Visual Backbones}


% \author{
% Yulin Wang$^1$\thanks{Equal contribution.\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \textsuperscript{\Envelope}Corresponding author.} \ \ \ \ 
% Yang Yue$^1$$^*$ \ \ \ \ 
% Rui Lu$^1$ \ \ \ \ 
% Tianjiao Liu$^2$ \ \ \ \ 
% Zhao Zhong$^2$\\
% Shiji Song$^1$ \ \ \ \ 
% Gao Huang$^{1,3}$ \!\textsuperscript{\Envelope}\\
% {\small$^1$Department of Automation, BNRist, Tsinghua University\ \ \ \ \ \ $^2$Huawei Technologies Ltd.}\\[-0.5ex]
% {\small$^3$Beijing Academy of Artificial Intelligence (BAAI)}\\
% {\small\texttt{\{wang-yl19, yueyang22, r-lu21\}@mails.tsinghua.edu.cn},}\\[-0.5ex]
% {\small\texttt{ \texttt{\{liutianjiao3, zorro.zhongzhao\}@huawei.com},\ \{shijis, gaohuang\}@tsinghua.edu.cn}}
% }


% \maketitle

% %%%%%%%%% ABSTRACT

% \newcommand{\gr}{\rowcolor[gray]{.9}}


% \begin{abstract}
%   The superior performance of modern deep networks usually comes at the price of a costly training procedure. In this paper, we present a novel curriculum learning approach for the efficient training of visual backbones (e.g., vision Transformers). The proposed method is inspired by the phenomenon that deep networks mainly learn to recognize some `easier-to-learn' discriminative patterns within each example at earlier stages of training, e.g., the lower-frequency components of images and the original information before data augmentation. Driven by this observation, we propose a curriculum where the model always leverages all the training data at each epoch, while the curriculum starts with only exposing the `easier-to-learn' patterns of each example, and introduces gradually more difficult patterns. To implement this idea, we 1) introduce a cropping operation in the Fourier spectrum of the inputs, which enables the model to learn from only the lower-frequency components efficiently, and 2) demonstrate that exposing the features of original images amounts to adopting weaker data augmentation. Our resulting algorithm, {EfficientTrain}, is simple, general, yet surprisingly effective. For example, it reduces the training time of a wide variety of popular models (e.g., ConvNeXts, DeiT, PVT, and Swin/CSWin Transformers) by more than $\bm{1.5\times}$ on ImageNet-1K/22K without sacrificing the accuracy. It is effective for self-supervised learning (i.e., MAE) as well. Code is available at \url{https://github.com/LeapLabTHU/EfficientTrain}.
% \end{abstract}


% \input{intro.tex}

% \input{related.tex}

% \input{method.tex}

% \input{experiment.tex}

% \input{conclusion.tex}


% \section*{Acknowledgements}

% % This work is supported in part by National Key R\&D Program of China (2020AAA0105200), the National Natural Science Foundation of China under Grants 62022048, and Guoqiang Institute of Tsinghua University. This work is also supported by Huawei Technologies Ltd. 
% This work is supported in part by National Key R\&D Program of China (2021ZD0140407), the National Natural Science Foundation of China under Grant 62022048, Guoqiang Institute of Tsinghua University and Huawei Technologies Ltd.


% {\small
% \bibliographystyle{ieee_fullname}
% \bibliography{IEEEtran}
% }

% \newpage
% \onecolumn
% \appendix

% \input{appendix.tex}


% \end{document}


==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************

